Enabling Reasoning with LegalRuleML

In order to automate verification process, regulatory rules written in natural language need to be translated into a format that machines can understand. However, none of the existing formalisms can fully represent the elements that appear in legal norms. For instance, most of these formalisms do not provide features to capture the behavior of deontic effects, which is an important aspect in automated compliance checking. This paper presents an approach for transforming legal norms represented using LegalRuleML to a variant of Modal Defeasible Logic (and vice versa) such that a legal statement represented using LegalRuleML can be transformed into a machine-readable format that can be understood and reasoned about depending upon the client's preferences.

==> Makefile <==

TARGETS=paper.pdf
EXTRAS=
PAPER_FILENAME=

###
### for images conversion from tex to png
###
# 1. installation of 'imagemagick' is needed for image conversion
IMAGES_FOLDER=images
# 2. additional latex packages/tikz libraries needed for images generation
LATEX_PACKAGES=../Latex/Macros/macros_commons ../Latex/Macros/macros_paper varwidth 
TIKZ_LIBS=decorations.text
###
###


include ./Makefile.inc

%.pdf: %.tex %.bbl
# uncomment the following lines for presentation handout
	# ${PDF} "\PassOptionsToClass{handout}{beamer}\input{$<}"
	# ${PDF} "\PassOptionsToClass{handout}{beamer}\input{$<}"
	# ${PDF} "\PassOptionsToClass{handout}{beamer}\input{$<}"
	# if [ "$@" ==  "${TARGETS}" ]; then  \
	# 	if [ "x${PAPER_FILENAME}" != "x" ]; then \
	# 		mv $@ ${PAPER_FILENAME:%.pdf=%_handout.pdf} ;\
	# 	else \
	# 		mv $@ ${@:%.pdf=%_handout.pdf} ;\
	# 	fi ;\
	# else \
	# 	mv $@ ${@:%.pdf=%_handout.pdf} ;\
	# fi
	${PDF} $<
	${PDF} $<
	if [ "$@" ==  "${TARGETS}" ]; then  \
		if [ "x${PAPER_FILENAME}" != "x" ]; then \
			cp "$@" "../${PAPER_FILENAME}" ;\
		fi ;\
	fi


==> content/bak/StatementsToRules.tex <==
%!TEX root = ../paper.tex

%==============================
% SEC: FROM LEGALRULEML TO DL
%==============================

% \ignore{\newpage}
% \mathchardef\text{-}="2D
\section{Mapping Legal RuleML Statements into Defeasible Logic Theory}
\label{sec:mapping}
The core of any Legal RuleML document revolves around the use of various key legal statements which include \emph{constitutive, prescriptive, factual, penalty, reparation} and \emph{override} statements. As such in order to map Legal RuleML into a DL theory, these statements are crucial in how they are defined in DL. 

\subsection{Modality Mapping}
\label{sec:modalityMapping}
Before we discuss how the various statements are mapped into DL rules, consideration of the mapping of various literal modalities in DL is required. Within Legal RuleML the various modality statements often contain ``Slot'' statements which usually contains the bearer and/or auxiliary party information. However, in DL this slot information is modelled by modifying the modality tag slightly, for example an obligation is modelled as $[\OBL]$ which when parsing a Legal RuleML document into DL theory the obligation statement becomes $[\OBL{:}Y{:}Y]$. This is best shown in \Cref{code:slot}, where the ``Right'' statement contains slot tags that contain bearer and auxiliary party information. After processing through the parser this statement would be mapped into the literal $ [RIGHT{:}Y{:}Y]rel2(X) $. Notice how the modality is modified to include the bearer and auxiliary party information by including a colon to differentiate the various sections. The first section is the standard modality tag indicating `RIGHT', the second section contains the bearer information in this case `Y', the final section contains the auxiliary party information which in this case is also `Y'. If either of the slot information is not present then the appropriate section is marked with the value `NULL'.

% \noindent\begin{minipage}{\textwidth}
\begin{lstlisting}[language=XML,float,
	,nolol=true
	,caption={Example Right Statement}
	,label=code:rightStatement,
	]
<lrml:Right>
    <ruleml:slot>
    	<lrml:Bearer />
		<ruleml:Var>Y</ruleml:Var>
    </ruleml:slot>
    <ruleml:slot>
    	<lrml:AuxiliaryParty />
        <ruleml:Var>Y</ruleml:Var>
    </ruleml:slot>
    <ruleml:Atom key="atom5">
    	<ruleml:Rel iri="rel2"/>
    	<ruleml:Var>X</ruleml:Var>
    </ruleml:Atom>
</lrml:Right>
\end{lstlisting}
% \end{minipage}

% \subsection{Constitutive Statements}
% \label{sec:constitutive}
% Consitutive statements contain constitutive rules, which define concepts or constitutive activities that cannot exist without such rules~\cite{OASISLRMLTC.2015}. These statements do not prescribe behaviours of any parties or activities involved and as such if these rules do not define any strength properties then the rules are mapped into DL as a strict rules, which indicates that these rules are indisputable. This is best shown in \Cref{code:constitutiveStatement}, where after parsing the constitutive statement would result in the following DL rule:   
% \[ \textnormal{ruletemplate1}:~A(X) \strict B(X) \]

% % \noindent\begin{minipage}{\textwidth}
% \begin{lstlisting}[language=XML,float,
% 	,nolol=true
% 	,caption={Example Constitutive Statement}
% 	,label=code:constitutiveStatement
% 	]
% <lrml:ConstitutiveStatement key="cs1">
% 	<ruleml:Rule key="ruletemplate1">
% 		<ruleml:if> 
% 			<ruleml:Atom>
%           		<ruleml:Rel>A</ruleml:Rel>
%                 <ruleml:Var>X</ruleml:Var>
%         	</ruleml:Atom>
%         </ruleml:if>
% 		<ruleml:then> 
% 			<ruleml:Atom>
%           		<ruleml:Rel>B</ruleml:Rel>
%                 <ruleml:Var>X</ruleml:Var>
%         	</ruleml:Atom>
%         </ruleml:then>
% 	</ruleml:Rule>
% </lrml:ConstitutiveStatement>
% \end{lstlisting}
% % \end{minipage}

% \subsection{Prescriptive Statements}
% \label{sec:prescriptive}
% Prescriptive statements contain prescriptive rules, which prescribes behaviours via regulating actions by making them obligatory, permitted, or prohibited~\cite{OASISLRMLTC.2015} along with the conditions in which these behaviours hold. When these prescriptive rules are mapped into DL the type of rule is defined as a defeasible rule, unless the prescriptive rule outlines any strength properties. This indicates that, in the absence of information to the contrary and where the rule holds, then the conclusion of the rule holds. After parsing the prescriptive statement in \Cref{code:prescriptivestatement2}, the result would be the following DL rule: 
% \[ \textnormal{ruletemplate2}:~rel1(X), [PER:Y:NULL] rel2(X) \defeasible \neg rel3(X) \]

% % \noindent\begin{minipage}{\textwidth}
% \begin{lstlisting}[language=XML,float,
% 	,nolol=true
% 	,caption={Example Prescriptive Statement}
% 	,label=code:prescriptivestatement2
% 	]
% <lrml:PrescriptiveStatement key="ps1">
% 		<ruleml:Rule key="ruletemplate2" closure="universal">
%     	<ruleml:if>
%       		<ruleml:And key="and1">
%         		<ruleml:Atom key="atom4">
%           			<ruleml:Rel iri="rel1"/>
%           			<ruleml:Var>X</ruleml:Var>
%         		</ruleml:Atom
%         		<lrml:Permission>
%         			<ruleml:slot>
% 			        	<lrml:Bearer />
% 						<ruleml:Var>Y</ruleml:Var>
% 			        </ruleml:slot>
%           			<ruleml:Atom key="atom4">
%            				<ruleml:Rel iri="rel2"/>
%             			<ruleml:Var>X</ruleml:Var>
%           			</ruleml:Atom>
%         		</lrml:Permission>
%       		</ruleml:And>
%    	 	</ruleml:if>
% 			<ruleml:then>
%   			<ruleml:Neg key="neg1">
%     			<ruleml:Atom key="atom6">
%       				<ruleml:Rel iri="rel3"/>
%       				<ruleml:Var>X</ruleml:Var>
%     			</ruleml:Atom>
%   			</ruleml:Neg>
% 		</ruleml:then>
% 		</ruleml:Rule>
% </lrml:PrescriptiveStatement>
% \end{lstlisting}
% % \end{minipage}


% \subsection{Factual Statements}
% \label{sec:fact}
% Factual statements in essence are the expression of fact and as such these statements are mapped into a DL rule with a fact rule type. In the absence of any temporal characteristics and jurisdiction information these rules hold true under all circumstances. The parsing of the factual statement in \Cref{code:fact} generates the following defeasible rule: 
% \[ \textnormal{fact1}:~\factrule rel5(JohnDoe) \]

% % \noindent\begin{minipage}{\textwidth}
% \begin{lstlisting}[language=XML,float,
% 	,nolol=true
% 	,caption={Example Factual Statement}
% 	,label=code:fact
% 	]
% <lrml:FactualStatement key="fact1">
% 	<lrml:hasTemplate>
% 		<ruleml:Atom key="atom11">
% 			<ruleml:Rel iri="rel5"/>
%       		<ruleml:Ind iri="JohnDoe"/>
%     	</ruleml:Atom>
%   	</lrml:hasTemplate>
% </lrml:FactualStatement>
% \end{lstlisting}
% % \end{minipage}

% \subsection{Penalty and Reparation Statements}
% \label{sec:penalty}
% In Legal RuleML the penalty statements represent a form of punishment, correction and/or repercussion for a violation of a specified rule as outlined in the reparation statement. In essence the reparation statement binds a penalty statement to the appropriate prescriptive statement. This penalty is applied if violation occurs of a deontic specification within the prescriptive statement. The penalty and reparation statements in \Cref{code:penalty} would result in the rule from prescriptive statement `ps1' having the literal $[\OBL:Y:NULL]rel6(X)$ applied as an additional literal on the head of the rule. If we use the `ps1' from \Cref{code:prescriptivestatement} as an example, then after parsing the resulting DL rule would be:
% % \begin{multline}
% \[
% \begin{array}{ll}
% \textnormal{ruletemplate2}: &  rel1(X), [PER:Y:NULL]rel2(X) \\
% 	& \qquad\qquad\defeasible \neg rel3(X), [OBL:Y:NULL]rel6(X)
% \end{array}
% \]
% % \end{multline}

% % \noindent\begin{minipage}{\textwidth}
% \begin{lstlisting}[language=XML,float,
% 	,nolol=true
% 	,caption={Example Penalty and Reparation Statements}
% 	,label=code:penalty
% 	]
% <lrml:PenaltyStatement key="pen1">
%   	<lrml:Obligation>
%   		<ruleml:slot>
%         	<lrml:Bearer />
% 			<ruleml:Var>Y</ruleml:Var>
%         </ruleml:slot>
%     	<ruleml:Atom key="atom9">
%       		<ruleml:Rel iri="rel6"/>
%       		<ruleml:Var>X</ruleml:Var>
%     	</ruleml:Atom>
%   	</lrml:Obligation>
% </lrml:PenaltyStatement>
% <lrml:ReparationStatement key="reps1">
%   	<lrml:Reparation key="rep1">
%     	<lrml:appliesPenalty keyref="#pen1"/>
%     	<lrml:toPrescriptiveStatement keyref="#ps1"/>
%   	</lrml:Reparation>
% </lrml:ReparationStatement>
% \end{lstlisting}
% % \end{minipage}

% \subsection{Override Statements}
% \label{sec:oerride}
% The override statement in Legal RuleML represents the \emph{superiority relation} used within DL. As DL does not support contradictory conclusions and instead seeks to resolve conflicts, in cases where there is some support for concluding A but also support for concluding B, DL does not conclude neither of them due to the confliction. However, if the support for A has priority over B then A is concluded~\cite{Lam.2009}. Therefore no conclusion can be drawn from conflicting rules in DL unless these rules are prioritised via superiority relations. In DL where one rule may override the conclusion of another, the superiority relation is used to define priorities amongst the rules. In essence the superiority relation provides information about the relative strength of rules over each other and only effects the proof theory if used for conflicting rules with complementary heads~\cite{Antoniou.2001}. For example, given animal `X' and the following facts:
% \begin{align}
% &\factrule bird(X) \nonumber \\
% &\factrule penguin(X) \nonumber
% \end{align}

% \noindent and the defeasible rules:
% \begin{align}
% r1 &: bird(X) \defeasible fly(X) \nonumber \\
% r2 &: penguin(X) \defeasible \neg fly(X) \nonumber
% \end{align}
% which contradict one another, no valid conclusion can be drawn about whether animal `X' is able to fly. However, if the superiority relation $r2 \superior r1 $ is included in the theory then we can conclude that animal `X' is unable to fly as penguin are unable to fly. \Cref{code:override} shows how a superiority relation is represented in an override statement within Legal RuleML where statement `ps2' overrides statement `ps1' $(ps2 \superior ps1 )$.

% % \noindent\begin{minipage}{\textwidth}
% \begin{lstlisting}[language=XML,float,
% 	,nolol=true
% 	,caption={Example Override Statement}
% 	,label=code:override
% 	]
% <lrml:OverrideStatement>
% 	<lrml:Override over="#ps2" under="#ps1"/>
% </lrml:OverrideStatement>
% \end{lstlisting}
% % \end{minipage}


\subsection{Mapping ``Or'' Statements}
\label{OrStatements}
Within Legal RuleML a rule can contain ``Or'' statements, which DL does not directly support. In order to map these statements into DL, these statements need to be considered as splitting the rule into multiple DL rules. As seen in \Cref{code:orStatement} the Prescriptive statement `ps2' contains rule `ruletemplate3'. This rule contains an ``Or'' statement which as mentioned above, this statement will be required to split into multiple DL rules based upon the amount of items within the ``Or'' statement. The naming convention used within the parser is that if a rule is split into multiple sub rules then each sub rule name contains the base rule name and is appended with a hyphen and a number that increments with each sub rule. This example in \Cref{code:orStatement}, after parsing would produce the following DL rules:
\begin{align}
ruletemplate3\text{-}1: &[PER:Y:NULL]rel1(X),[OBL:NULL:NULL]rel2(X) \defeasible \nonumber \\ &[PRO:NULL:NULL] rel3(X)
\nonumber \\
ruletemplate3\text{-}2: &[PER:Y:NULL]rel1(X),[RIGHT:Y:Y]rel2(X) \defeasible \nonumber \\ &[PRO:NULL:NULL] rel3(X) \nonumber
\end{align}

% \noindent\begin{minipage}{\textwidth}
\begin{lstlisting}[language=XML,float,
	,nolol=true
	,caption={Example Or Statement}
	,label=code:orStatement
	]
<lrml:PrescriptiveStatement key="ps2">
	<ruleml:Rule key="ruletemplate3" closure="universal">
	<ruleml:if>
		<ruleml:And key="and1">
			<lrml:Permission>
				<ruleml:slot>
		        	<lrml:Bearer />
					<ruleml:Var>Y</ruleml:Var>
		        </ruleml:slot>
	            <ruleml:Atom key="atom4">
	            	<ruleml:Rel iri="rel1"/>
	                <ruleml:Var>X</ruleml:Var>
	            </ruleml:Atom>
			</lrml:Permission>
			<ruleml:Or key="or1">
  				<lrml:Obligation key="oblig1">
    				<ruleml:Atom key="atom5">
      					<ruleml:Rel iri="rel2"/>
      					<ruleml:Var>X</ruleml:Var>
    				</ruleml:Atom>
  				</lrml:Obligation>
  				<lrml:Right>
  					<ruleml:slot>
			        	<lrml:Bearer />
						<ruleml:Var>Y</ruleml:Var>
			        </ruleml:slot>
			        <ruleml:slot>
			        	<lrml:AuxiliaryParty />
						<ruleml:Var>Y</ruleml:Var>
			        </ruleml:slot>
    				<ruleml:Atom key="atom5">
      					<ruleml:Rel iri="rel2"/>
      					<ruleml:Var>X</ruleml:Var>
    				</ruleml:Atom>
  				</lrml:Right>
			</ruleml:Or>
		</ruleml:And>
	</ruleml:if>
    <ruleml:then>
      	<lrml:Prohibition key="prohib1">
      		<ruleml:Atom key="atom6">
        		<ruleml:Rel iri="rel3"/>
        		<ruleml:Var>X</ruleml:Var>
      		</ruleml:Atom>
      	</lrml:Prohibition>
    </ruleml:then>
	</ruleml:Rule>
</lrml:PrescriptiveStatement>
\end{lstlisting}
% \end{minipage}


\subsection{Mapping ``And'' Statements in the Head of a Rule}
\label{sec:AndStatement}
Inside Legal RuleML rules there is the possibilities of ``And'' statements which are handled differently depending on if they occur in the body or the head of a rule. If the ``And'' statement occur in the body of a Legal RuleML rule then each literal is appended to the body of the DL rule. An ``And'' statement within the head of a rule indicates the combination of multiple literals is required. However, DL theory does not provide direct functionality for this and as such these ``And'' statements are mapped into multiple rules. As discussed in \Cref{OrStatements}, the parser naming convention uses a hyphen and a number to distinguish each split from the base rule, which is also used for splits occurring due to an ``And'' statement. However, if the rule is all ready a sub rule then further splitting is required for each previously split rule. The parser naming convention when a further split is required, is after the incrementing number a alphabet character a-z is used. An example of this in \Cref{code:andStatement} would result in the following DL rules where `a' and `b' are appended to each split rule:
\begin{align}
ruletemplate3\text{-}1a: &[Per:Y:Null]rel1(X),[Obl:Null:Null]rel2(X) \defeasible \nonumber \\
&[Pro:Null:Null] rel3(X), rel4(X) 
\nonumber \\ 
ruletemplate3\text{-}1b: &[PER:Y:NULL]rel1(X),[OBL:NULL:NULL]rel2(X) \defeasible \nonumber \\
&[PRO:NULL:NULL] rel3(X), [OBL:NULL:NULL]rel5(X)
\nonumber \\ 
ruletemplate3\text{-}2a: &[PER:Y:NULL]rel1(X),[RIGHT:Y:Y]rel2(X) \defeasible \nonumber \\
&[PRO:NULL:NULL] rel3(X), rel4(X)
\nonumber \\ 
ruletemplate3\text{-}2b: &[PER:Y:NULL]rel1(X),[RIGHT:Y:Y]rel2(X) \defeasible \nonumber \\
&[PRO:NULL:NULL] rel3(X), [OBL:NULL:NULL]rel5(X) \nonumber
\end{align}

% \noindent\begin{minipage}{\textwidth}
\begin{lstlisting}[language=XML,float=t,
	,nolol=true
	,caption={Example And Statement}
	,label=code:andStatement
	]
<lrml:PrescriptiveStatement key="ps2">
		<ruleml:Rule key="ruletemplate4" keyref="ruletemplate3">
        <ruleml:then>
          	<lrml:SuborderList>
	            <lrml:Prohibition key="prohib2">
	              	<ruleml:Atom key="atom26">
	                	<ruleml:Rel iri="rel3"/>
	                	<ruleml:Var>X</ruleml:Var>
	              	</ruleml:Atom>
	            </lrml:Prohibition>
	            <ruleml:And>
	            	<ruleml:Atom key="atom27">
	                	<ruleml:Rel iri="rel4"/>
	                	<ruleml:Var>X</ruleml:Var>
	              	</ruleml:Atom>
	              	<lrml:Obligation key="ob1">
	                	<ruleml:Atom key="atom28">
	                  		<ruleml:Rel iri="rel5"/>
	                  	<ruleml:Var>X</ruleml:Var>
	                	</ruleml:Atom>
	              	</lrml:Obligation>
	            </ruleml:And>
	        </lrml:SuborderList>
        </ruleml:then>
	</ruleml:Rule>
</lrml:PrescriptiveStatement>
\end{lstlisting}
% \end{minipage}

\subsection{Violation and Compliance statements}
\label{sec:contraryToDuty}
Within Legal RuleML rules there can be ``Violation'' and ``Compliance'' statements, which refer to an obligation or prohibition literal inside the document. A violation statement indicates that the contents of the literal referred to has not been met, as it has been violated. The compliance statement represents that either the referred Obligation has been fulfilled or the referred Prohibition has not been violated. When mapped to DL, these statements are best represented by replacing the reference to the obligation or prohibition literal with two new literals in the rule. These new literals vary depending on the modality as well as if it is a violation or compliance. This is best shown by the following example: 

\begin{enumerate}
  \item Violation
  \begin{enumerate}
    \item $[OBL]a$: Obligation of `a' becomes $[OBL]\neg a, \neg a$
    \item $[PRO]b$: Prohibition of `b' becomes $[PRO]\neg a, a$
  \end{enumerate}
  \item Compliance
  \begin{enumerate}
    \item $[OBL]a$: Obligation of `a' becomes $[OBL] a, a$
    \item $[PRO]b$: Prohibition of `b' becomes $[PRO] a, \neg a$
  \end{enumerate}
\end{enumerate}

% \ignore{\newpage}



==> content/bak/otherInformation.tex <==
%!TEX root = ../paper.tex
\section{Refine Defeasible Logic Theory by Requirement}
\label{sec:byRequirement}
Within a Legal RuleML document further information may be present that is not required for the reasoning process performed by DL. However, this information may be required under certain circumstances, for example under particular jurisdiction requirements. Additional functionality within the theory has been implemented to return a subtheory containing only the information relevant to the chosen jurisdiction requirement. 

\subsection{Refine Defeasible Logic Theory by Jurisdiction}
If reasoning on a Legal RuleML document is required based upon particular jurisdiction requirements then functionality has been included to return a subtheory of all data within the specified jurisdiction. This subtheory only contains the rules, superiority relations and supporting information that relates to the chosen jurisdiction, unless the Legal RuleML document contains rules that are flagged with a universal closure. Universal closure indicates that the rule holds under all jurisdictions. For example, a Legal RuleML document represents a particular law that some rules are only enforced in certain jurisdictions or states within a country and these rules may even conflict with other rules for other states. Therefore the subtheory created will only contain the rules for the particular state requested to be reasoned. As seen in~\Cref{code:jurisdiction} the association `asn-ps3' applies jurisdiction of Italy and contains ``appliesSource'' and ``appliesModality'' information which applies to the target statement `ps3'. This shows that under the jurisdiction of Italy this rule `ps3' has a defeater strength, which outside this jurisdiction would be classified with a defeasible strength. However, as seen in statement `ps4', the rule labelled `ruletemplate4' indicates a universal closure which would also be present within the subtheory created by jurisdictions requirement of Italy. 

% \noindent\begin{minipage}{\textwidth}
\begin{lstlisting}[language=XML,float,
	,nolol=true
	,caption={Example Jurisdiction and Association Statements}
	,label=code:jurisdiction
	]
<?xml version="1.0" encoding="UTF-8" standalone="yes"?>
<lrml:LegalRuleML>
	...
	<!-- Jurisdictions -->
  	<lrml:Jurisdictions>
    	<lrml:Jurisdiction key="italy" sameAs="http://example.org/jurisdiction#italy"/>
  	</lrml:Jurisdictions>
  	...
  	<!-- Associations -->
	<lrml:Associations  key="asn-1">
    	<lrml:Association key="asn-ps3">
      		<lrml:appliesSource keyref="#ex-ref1"/>
      		<lrml:appliesModality iri="http://spin.nicta.com.au/spindle/ruleStrength#defeater"/>
      		<lrml:appliesJurisdiction keyref="#italy"/>
      		<lrml:toTarget keyref="#ps3"/>
    	</lrml:Association>
  	</lrml:Associations>
	<lrml:Statements>
		...
		<lrml:PrescriptiveStatement key="ps3">
			<ruleml:Rule key="ruletemplate3">
				<ruleml:if> ... </ruleml:if>
				<ruleml:then> ... </ruleml:then>
			</ruleml:Rule>
		</lrml:PrescriptiveStatement>
		<lrml:PrescriptiveStatement key="ps4">
			<ruleml:Rule closure="universal" key="ruletemplate4">
				<ruleml:if> ... </rulfeml:if>
				<ruleml:then> ... </ruleml:then>
			</ruleml:Rule>
		</lrml:PrescriptiveStatement>
        ...
	</lrml:Statements>
	...
</lrml:LegalRuleML>
\end{lstlisting}
% \end{minipage}
